Differentially Private Stream Processing at Scale

We design, to the best of our knowledge, the first differentially private (DP) stream aggregation processing system at scale. Our system -- Differential Privacy SQL Pipelines (DP-SQLP) -- is built using a streaming framework similar to Spark streaming, and is built on top of the Spanner database and the F1 query engine from Google. Towards designing DP-SQLP we make both algorithmic and systemic advances, namely, we (i) design a novel (user-level) DP key selection algorithm that can operate on an unbounded set of possible keys, and can scale to one billion keys that users have contributed, (ii) design a preemptive execution scheme for DP key selection that avoids enumerating all the keys at each triggering time, and (iii) use algorithmic techniques from DP continual observation to release a continual DP histogram of user contributions to different keys over the stream length. We empirically demonstrate the efficacy by obtaining at least $16\times$ reduction in error over meaningful baselines we consider. We implemented a streaming differentially private user impressions for Google Shopping with DP-SQLP. The streaming DP algorithms are further applied to Google Trends.

==> intro.tex <==
\section{Introduction}
\label{sec:intro}

Analysis of streaming data with differential privacy (DP)~\cite{DMNS} has been studied from the initial days of the field~\cite{Dwork-continual,CSS11-continual}, and this has been followed up in a sequence of works that include computing simple statistics~\cite{perrier2018private}, to machine learning applications (a.k.a.,~online learning)~\cite{JKT-online,thakurta2013nearly,agarwal2017price,kairouz2021practical,erlingsson2019private}. While all of these works focus on the abstract algorithmic design for various artifacts of streaming data processing, to the best of our knowledge, none of them focus on designing a scalable stream processing system. In this work, we primarily focus on designing a scalable DP stream processing system, called Differential Privacy SQL Pipelines (DP-SQLP), and make algorithmic advances along the way to cater to the scalability needs of it. DP-SQLP is implemented using a streaming framework similar to Spark streaming~\cite{Zaharia13streamingspark}, and is built on top of the Spanner database~\cite{corbett2013spanner} and F1 query engine~\cite{samwel2018f1} from Google.

\mypar{Motivation} In this paper we consider a data stream to be an unbounded sequence of tuples of the form $(\recordkey,$ $\recordvalue,$ $\recordtimestamp,$ $\recorduserid)$ that gets generated continuously in time. These data streams appear naturally in various settings like Web logs, spatio-temporal GPS traces~\cite{andres2013geo}, mobile App usages~\cite{latif2020introducing}, data generated by sensor networks and smart devices~\cite{liu2018epic}, live traffic in maps~\cite{wang2016differential}, cardiovascular monitoring~\cite{tan2021toward}, real-time content recommendation~\cite{phelan2009using}, and pandemic contact tracing~\cite{cho2020contact}. Almost all of these applications touch sensitive user data on a continual basis.~\cite{Calandrino11-like} demonstrated that continuous data release about individuals can act as a strong attack vector for detecting the presence/absence of a single user (in the context of collaborative recommendation systems). Hence, it is imperative to a streaming system to have rigorous privacy protections. In this work we adhere to differential privacy. For more discussion on the type of streams we consider, see a detailed survey in~\cite{isah2019survey}.

\mypar{DP and its challenges in stream processing} Differential privacy %
provides a formal guarantee about how much the output of an algorithm reveals about any individual in its input \cite{DMNS,dwork2014algorithmic}. Although prior research has extended simple one-shot DP algorithms to the streaming setting \cite{Dwork-continual,CSS11-continual,cardoso2022differentially}, in the area of data processing, most DP deployments focus on one-shot batch processing \cite{wilson2019differentially,appledp,amin2022plume}. %

There are many challenges when applying differential privacy to stream processing systems. The three main obstacles are:
\begin{enumerate}[label=(\roman*)]
    \item One-shot DP algorithms \cite{wilson2019differentially,mcsherry2007mechanism} cannot be directly applied to stream processing, due to privacy budget constraints. If we apply a DP algorithm repeatedly, the privacy cost rapidly accumulates. Said differently, if we apply DP mechanisms (e.g., exponential mechanism~\cite{mcsherry2007mechanism}) many times, the noise must be extremely large. Furthermore, some one-shot DP algorithms (e.g., key selection \cite{wilson2019differentially}) do not support incremental release. 
    \item In real applications, each person may contribute multiple records to the data stream at different times. Providing ``event-level DP'' (where a single action by a person/user is protected) does not provide sufficient privacy protection. In this work, we provide ``user-level DP'', where~\emph{all} the actions by a person/user is protected. %
    \item A data stream processing system is naturally driven by the input data stream. It can only process the data that has arrived. We refer to the times when our system runs as \emph{triggering times}. For example, keys for a $\groupby$ operation are not known in advance; instead we discover new keys as they arrive. The input-driven nature of our system presents an unavoidable limitation for privacy, as the triggering times may leak information; we will discuss this limitation more later.
\end{enumerate}

\mypar{Motivation} Data streams are sequences of unbounded tuples generated continuously in time (see the survey~\cite{isah2019survey}), such as Web logs, spatial-temporal GPS traces, mobile App usages, and data generated by sensor networks and smart devices. The ability to process data streams in real-time and continuously release results is critical for many applications used in our daily life, from navigation with live traffic to cardiovascular monitoring~\cite{tan2021toward}, and from real-time content recommendation to pandemic contact tracing. However, many of these data streams may contain sensitive personal information. Therefore, it is critical for applications to adopt privacy preserving technologies and ensure no individual information could be revealed from released real-time data.\anote{Need way more citation. An important system as this cannot be studied only in two papers :)}

\mypar{Our contributions at a glance} Our main contribution in this paper is:
\begin{center}
    \emph{We provide the first at-scale differentially private distributed stream processing system (a.k.a. DP-SQLP).}
\end{center}
In the following, we describe the algorithmic and systemic innovations that were required to realize the DP-SQLP system.
\begin{enumerate}
    \item As discussed earlier, we are dealing with an input-driven system, which is typical for any distributed streaming systems~\cite{Zaharia13streamingspark,akidau2015dataflow,DBLP:CarboneKEMHT15flink}. Hence, the time at which data processing occurs heavily depends on when a user contributes. This complicates the information we can hope to protect via DP. To that end, we propose a formal notion of data set neighborhood (in Definition~\ref{def:neighbors}) that allows us to formally capture the information we \emph{can} protect in a practical streaming system.
    
    \item  For each $\recordkey$ encountered in the data stream, the objective is to continually release the number of user records contributed to that key at regular time intervals. There are two challenges that arise in the context of DP: (a) The existence of $\recordkey$ is only known when it is observed in a user data record, and (b) the information leakage due to continually releasing the information about any particular key increases the DP cost due to composition~\cite{dwork2014algorithmic}. To address the first challenge, we design a new algorithm (Algorithm~\ref{Alg:key-selection}) that couples ``binary tree aggregation''~\cite{Dwork-continual,CSS11-continual,honaker2015efficient} (a standard tool for continual data release with DP) with a novel thresholding scheme that allows one to operate with keys that have at least $\mu>0$ user records with them. To address the second concern, we resort to a variance reduced implementation of the binary tree aggregation protocol~\cite{honaker2015efficient} that only accumulates privacy cost that is poly-logarithmic in the number of aggregate releases from the data stream.
    \item In a real system, since the potential key space is far too large to scan through, it is not scalable to load all keys each time the system is invoked. We design a new algorithm (Algorithm~\ref{Alg:empty-key-prediction}) that allows only checking for keys that have appeared between two consecutive triggering timestamps. When determining the condition of data release, we make a prediction for the future time. By doing so, we reduced the expensive I/O and memory cost, with a little CPU overhead.
    \item We provide a thorough empirical evaluation of our system. We consider a few natural baselines that adopt one-shot DP algorithms in stream data processing (e.g., repeated differential privacy query). We observed up to 94.8\% error reduction and the number of retained keys is increased by 4633 times when comparing DP-SQLP with baselines.
\end{enumerate}

In the following, we formally define the problem, and delve deeper into relevant related works.

\subsection{Problem Statement}
Let $D$ be a data stream defined by a sequence of infinite records, i.e., $D=[d_1, d_2,...)$, where each record $d_i$ is a tuple 
$(\recordkey,$ $\recordvalue,$ $\recordtimestamp t_i,$ $\recorduserid)$. A common query pattern in data analytics is the unknown domain histogram query. For example, consider a web service that logs user activities: each record is a URL click that contains $(\texttt{URL},$ $\recorduserid,$ $\recordtimestamp)$. An analyst wants to know the number of clicks of URLs per-day, with latest update. A query to get the histogram is presented in Listing~\ref{target-sql1}.
\\

\begin{lstlisting}[
           language=SQL,
           showspaces=false,
           basicstyle=\ttfamily,
           numberstyle=\tiny,
           commentstyle=\color{gray},
           caption=Single histogram query,
           captionpos=b,
           label=target-sql1,
           frame=single
        ]
SELECT URL, 
       TO_DATE(timestamp) AS date, 
       COUNT(*) AS count
FROM web_logs
GROUP BY URL, TO_DATE(timestamp)
\end{lstlisting}

In Listing \ref{target-sql1}, the keys are $(\texttt{URL}, \texttt{date})$ denoted by $k$, and the $\texttt{count}$ is an aggregation column denoted by $m$. 

When querying a growing database or data stream, the above-mentioned query only shows a snapshot at certain date. In stream data processing, there are commonly windowing semantics that determines what records in~\emph{event time domain} to process, and triggering semantics, that defines when in~\emph{processing time domain} the results of groupings are emitted \cite{akidau2015dataflow}.
Let $W$ denote the event-time windows, $W=[w_1, w_2...)$. Each event-time window is defined by a starting timestamp and end timestamp $w=(t_s, t_e)$. $D_w \in D$ contains all records that can be assigned to window $w$ so that $t_i$ of each record satisfies $t_s \leq t_i < t_e$. The streaming system incrementally processes records for a window, and the computations are triggered at a predefined set of timestamps $\tr = [t^{\sf tr}_1, t^{\sf tr}_2,...,t^{\sf tr}_T]$ for each window. Here, $t^{\sf tr}_T$ may be greater than $t_e$ due to the time domain skew\cite{akidau2015dataflow}. Our goal is to release the histogram for all sub-stream $D_w$, at every triggering timestamp $t^{\sf tr}_i$, in a differentially private (DP) manner. (See Section~\ref{sec:dpdef} for a formal DP definition.) For a pictorial representations of various timing concepts, see Figure~\ref{fig:time-domain}.

\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{pic/time-domains.png}
\caption{Event time domain and processing time domain}
\label{fig:time-domain}
\end{figure}






\subsection{Related Works}
Stream processing has been an active research field for more than 20 years~\cite{fragkoulis2020survey}. It is now considered to be a mature technology with various streaming frameworks deployed at scale in industry, including Spark Streaming~\cite{Zaharia13streamingspark}, Apache Beam~\cite{akidau2015dataflow} and Apache Flink~\cite{DBLP:CarboneKEMHT15flink}. However, none of these systems offer differentially private streaming queries.

Our work builds on a long line of DP research that focuses on extending one shot applications of DP mechanisms to the continual observation (streaming) setting for both analytics and learning applications \cite{Dwork-continual,CSS11-continual,honaker2015efficient, cardoso2022differentially, kairouz2021practical, li2015matrix, denisov2022improved, henzinger2022constant}. These mechanisms crucially leverage the tree aggregation protocol \cite{Dwork-continual,CSS11-continual,honaker2015efficient} or variants of it based on the matrix factorization mechanism \cite{li2015matrix, denisov2022improved, henzinger2022constant}. All these approaches have the advantage of drastically reducing the error induced by repeated application of a DP mechanism, making the DP protocol itself stateful. 

Of the above cited, our work is most related to \cite{cardoso2022differentially}, which investigates the problem of computing differentially private (unknown-domain) histograms under continual observations. Similar to our work, \citep{cardoso2022differentially} leverages (extensions of) the tree aggregation protocol \cite{Dwork-continual,CSS11-continual,honaker2015efficient} to build an efficient DP protocol for the continuous observation privacy setting. However, our work departs from theirs in a few fundamental ways: (a) we consider user level DP whereas they consider event level DP (this introduces interesting algorithmic and system challenges), (b) we provide a concrete streaming system architecture for scalable production deployments whereas they focus on developing algorithms (more precisely, we have an empty key prediction scheme that allows us to scale to one billion keys), and (c) we test our algorithms and architecture on a number of large-scale synthetic and real-life datasets to demonstrate the efficacy of our approach relative to meaningful baselines (experiments are completely absent from \cite{cardoso2022differentially}).  

\subsection{Organization}

The rest of the paper is organized as follows. In Section~\ref{sec:preliminaries} we provide the necessary background on differential privacy, and streaming systems; in Section~\ref{sec:sdp-overview} we describe the main algorithmic components of our DP streaming system; in Section~\ref{sec:streamingdpimp} we provide details of the systemic advanced needed to scale up the algorithms to large workloads; in Section~\ref{sec:experiments} we provide thorough empirical evaluation; and finally in Section~\ref{sec:conclusion} we provide some concluding remarks.




